From Imitation to Exploration: End-to-end Autonomous Driving based on World Model

In recent years, end-to-end autonomous driving architectures have gained increasing attention due to their advantage in avoiding error accumulation. Most existing end-to-end autonomous driving methods are based on Imitation Learning (IL), which can quickly derive driving strategies by mimicking expert behaviors. However, IL often struggles to handle scenarios outside the training dataset, especially in high-dynamic and interaction-intensive traffic environments. In contrast, Reinforcement Learning (RL)-based driving models can optimize driving decisions through interaction with the environment, improving adaptability and robustness. To leverage the strengths of both IL and RL, we propose RAMBLE, an end-to-end world model-based RL method for driving decision-making. RAMBLE extracts environmental context information from RGB images and LiDAR data through an asymmetrical variational autoencoder. A transformer-based architecture is then used to capture the dynamic transitions of traffic participants. Next, an actor-critic structure reinforcement learning algorithm is applied to derive driving strategies based on the latent features of the current state and dynamics. To accelerate policy convergence and ensure stable training, we introduce a training scheme that initializes the policy network using IL, and employs KL loss and soft update mechanisms to smoothly transition the model from IL to RL. RAMBLE achieves state-of-the-art performance in route completion rate on the CARLA Leaderboard 1.0 and completes all 38 scenarios on the CARLA Leaderboard 2.0, demonstrating its effectiveness in handling complex and dynamic traffic scenarios. The model will be open-sourced upon paper acceptance at https://github.com/SCP-CN-001/ramble to support further research and development in autonomous driving.

==> tables/annotation.tex <==
\begin{table}[htb]
    \centering
    \caption{}
    \begin{tabular}{l l} \toprule[2pt]
        \textbf{Annotation} & \textbf{Description} \\ \midrule
        t & Time \\
        $o_t$ & Raw sensor inputs at time $t$ \\
        $x_t$ & The ground truth semantic segmentation at time $t$ \\
        $\hat{x}_t$ & The estimated semantic segmentation at time $t$ \\
        $a_t$ & The action taken at time $t$
        \\ \bottomrule[2pt]
    \end{tabular}
\end{table}

==> tables/config-c-model.tex <==
\begin{table}
    \centering
    \caption{Hyper-parameters of SAC}
    \begin{tabular}{l l}
        \toprule[2pt]
        \textbf{Hyper-parameter} & \textbf{Value} \\
        \midrule
        State dimension & 2068 \\
        Hidden dimension & 1024 \\
        Action dimension & 2 \\
        $\gamma$ & 0.95 \\
        $\tau$ & 0.001 \\
        Learning rate & 0.0001 \\
        Initial temperature & 0.1 \\
        Target entropy & -2.0 \\
        Replay buffer size & 1000000 \\
        Warm-up steps & 10000 \\
        \bottomrule[2pt]
    \end{tabular}
\end{table}

==> tables/config-m-model.tex <==
\begin{table}
    \centering
    \caption{Hyper-parameters of the Transformer}
    \begin{tabular}{l l}
        \toprule[2pt]
        \textbf{Hyper-parameter} & \textbf{Value} \\
        \midrule
        Stochastic dimension & 1024 \\
        Action dimension & 3 \\
        Feature dimension & 1024 \\
        Key dimension & 1024 \\
        Value dimension & 1024 \\
        Hidden dimension & 2048 \\
        Layer number & 2 \\
        Head number & 8 \\
        Max length & 64 \\
        Dropout rate & 0.1 \\
        \bottomrule[2pt]
    \end{tabular}
\end{table}

\begin{table}
    \centering
    \caption{Dimension of the MLP Predictors}
    \begin{tabular}{l l}
        \toprule[2pt]
        \textbf{MLP} & \textbf{Dimension} \\
        \midrule
        Reward predictor & [1024, 1024, 4] \\
        Terminal predictor & [1024, 1024, 1] \\
        Dynamics predictor & [1024, 1024, 1024] \\
        \bottomrule[2pt]
    \end{tabular}
\end{table}

==> tables/config-sensor.tex <==
\begin{table}[htb]
    \centering
    \caption{The configured sensor's location with respect to the center of the ego vehicle.}
    \label{table: sensor-configuration}
    \begin{tabular}{l|c c c c c c c}
    \toprule[2pt]
        \textbf{Sensor} & x & y & z & roll & pitch & yaw & FOV \\ \midrule
        Camera (front) & 0.2 & 0.0 & 1.8 & 0$^{\circ}$ & 0$^{\circ}$ & 0$^{\circ}$ & 120$^{\circ}$ \\
        Camera (left) & -0.1 & -0.4 & 1.8 & 0$^{\circ}$ & -15$^{\circ}$ & -90$^{\circ}$ & 120$^{\circ}$ \\
        Camera (right) & -0.1 & 0.4 & 1.8 & 0$^{\circ}$ & -15$^{\circ}$ & 90$^{\circ}$ & 120$^{\circ}$ \\
        Camera (rear) & -0.5 & 0.0 & 1.8 & 0$^{\circ}$ & 0$^{\circ}$ & 180$^{\circ}$ & 120$^{\circ}$ \\
        LiDAR & 0.0 & 0.0 & 1.8 & 0$^{\circ}$ & 0$^{\circ}$ & 0$^{\circ}$ & 360$^{\circ}$ \\
        IMU & 0.0 & 0.0 & 0.0 & 0$^{\circ}$ & 0$^{\circ}$ & 0$^{\circ}$ & - \\
        GPS & 0.0 & 0.0 & 0.0 & 0$^{\circ}$ & 0$^{\circ}$ & 0$^{\circ}$ & - \\
        \bottomrule[2pt]
    \end{tabular}
\end{table}

==> tables/config-v-model.tex <==
\begin{table}[htb]
    \centering
    \caption{Hyper-parameters of SwinTransformer}
    \begin{tabular}{l  l}
        \toprule[2pt]
        \textbf{Hyper-parameter} & \textbf{Value} \\
        \midrule
        Embed dimension & 96 \\
        Depth & [2, 2, 6, 2] \\
        Header number & [3, 6, 12, 24] \\
        Window size & 7 \\
        MLP ratio & 4.0 \\
        QKV bias & True \\
        Hidden dropout & 0.0 \\
        Attention dropout & 0.0 \\
        Drop path rate & 0.3 \\
        \bottomrule[2pt]
    \end{tabular}
\end{table}

\begin{table}[htb]
    \centering
    \caption{Hyper-parameters of the Feature Pyramid Network}
    \begin{tabular}{l  l}
        \toprule[2pt]
        \textbf{Hyper-parameter} & \textbf{Value} \\
        \midrule
        Input channels & [192, 384, 768] \\
        Output channels & 256 \\
        Normalization & BatchNorm2d \\
        \bottomrule[2pt]
    \end{tabular}
\end{table}

\begin{table}
    \centering
    \caption{Hyper-parameters of the PointPillars Encoder (Point Feature Network)}
    \begin{tabular}{l  l}
        \toprule[2pt]
        \textbf{Hyper-parameter} & \textbf{Value} \\
        \midrule
        Input channels & 3 \\
        Feature channels & [128, 128] \\
        Normalization & True \\
        \bottomrule[2pt]
    \end{tabular}
\end{table}

\begin{table}
    \centering
    \caption{Hyper-parameters of the PointPillars Encoder (Scatter Network)}
    \begin{tabular}{l  l}
        \toprule[2pt]
        \textbf{Hyper-parameter} & \textbf{Value} \\
        \midrule
        Input channels & 128 \\
        Output shape & [128, 128] \\
        \bottomrule[2pt]
    \end{tabular}
\end{table}

\begin{table}
    \centering
    \caption{Hyper-parameters of the VAE}
    \begin{tabular}{l  l}
        \toprule[2pt]
        \textbf{Hyper-parameter} & \textbf{Value} \\
        \midrule
        Encoder channels & [32, 64, 128, 256] \\
        Decoder channels & [256, 128, 64, 32] \\
        Flatten dimension & [256, 16, 16] \\
        Latent dimension & 1024 \\
        \bottomrule[2pt]
    \end{tabular}
\end{table}


==> tables/result-efficiency-comparison.tex <==
\begin{table}[htb]
    \centering
    \caption{Efficiency comparison in CARLA Leaderboard}
    \label{efficiency_comparison}
    \begin{tabular}{l|cccc}\toprule[2pt]
        & \multicolumn{4}{c}{\textbf{Running}} \\ \cmidrule{2-5}
        \textbf{Method}  & \textbf{Average step} & \textbf{Average speed} & \textbf{Memory} & \textbf{GPU} \\
        &  ms, $\downarrow$ & m/s, $\uparrow$ & GB, $\downarrow$ & GB, $\downarrow$ \\ \midrule
        Roach \cite{zhang2021end} &  \\
        PDM-Lite \cite{renz2024carllava} & & 10 & 0 \\ \midrule
        LAV \cite{chen2022learning} \\
        TF++ WP \cite{jaeger2023hidden} \\
        TCP \cite{wu2022trajectory} \\ \midrule
        Ramble (Ours) \\ \bottomrule[2pt]
    \end{tabular}
\end{table}

==> tables/result-performance.tex <==
\begin{table*}[!htbp]

\centering
\caption{Performance comparison in CARLA Leaderboard 1.0}
\label{table: performance-L10}
\setlength\tabcolsep{4pt}

{\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccc|ccccccccc} \toprule[2pt]
\textbf{Method} & \textbf{RC} & \textbf{DS} & \textbf{IS} & \makecell{\textbf{Collisions}\\\textbf{pedestrians}} & \makecell{\textbf{Collisions}\\\textbf{vehicles}} & \makecell{\textbf{Collisions}\\\textbf{layout}} & \makecell{\textbf{Red light}} & \makecell{\textbf{Stop sign}} & \makecell{\textbf{Off-road}} & \makecell{\textbf{Agent}\\\textbf{blocked}} & \makecell{\textbf{Route}\\\textbf{deviations}} & \makecell{\textbf{Route}\\\textbf{timeout}} \\ \hline
& \%, $\uparrow$ & \%, $\uparrow$ & $\uparrow$ & \#/km, $\downarrow$ & \#/km, $\downarrow$ & \#/km, $\downarrow$ & \#/km, $\downarrow$ & \#/km, $\downarrow$ & \#/km, $\downarrow$ & \#/km, $\downarrow$ & \#/km, $\downarrow$ & \#/km, $\downarrow$ \\ \hline
Roach-RL \cite{zhang2021end} & 96.9 & 87.3 & 0.90 & 0.00 &  0.16 & 0.01 & 0.00 & 0.02 & 0.00 & 0.11 & 0.00 & 0.03 \\
Think2Drive$^*$ \cite{li2024think2drive} & 99.7 & 90.2 & - & - & - & - & - & - & - & - & - & - \\ \hline
ReasonNet$^*$ \cite{shao2023reasonnet} & 89.9 & \textbf{80.0} & \textbf{0.89} & 0.02 & 0.13 & 0.01 & 0.08 & 0.00 & 0.04 & 0.33 & 0.00 & 0.01 \\
LAV \cite{chen2022learning} & 84.2 & 54.4 & 0.67 & 0.00 & 0.27 & 0.16 & 0.04 & 0.62 & 0.05 & 0.12 & 0.32 & 0.14 \\
TransFuser++ \cite{jaeger2023hidden} & 97.2 & 70.9 & 0.73 & 0.00 & 0.24 & 0.15 & 0.05 & 0.36 & 0.07 & 0.09 & 0.00 & 0.06 \\
TCP \cite{wu2022trajectory} & 88.6 & 52.8 & 0.58 & 0.00 & 0.44 & 0.84 & 0.07 & 0.50 & 0.17 & 0.62 & 0.00 & 0.07 \\ \hline
Ramble (Ours) & \textbf{98.2} & 39.4 & 0.40 & 0.04 & 0.37 & 0.02 & 1.76 & 0.35 & 0.06 & 0.02 & 0.00 & 0.00 \\ \bottomrule[2pt]
\end{tabular}
}

\vspace{0.1cm}
\scriptsize
\textit{Notes}:
Roach-RL and Think2Drive are expert models having access to privileged information from the simulator's backend. The methods marked with $*$ are not open-source, and the testing reports are sourced from their original papers.

\vspace{0.5cm}

\caption{Performance of RAMBLE in the 38 scenarios intercepted from CARLA Leaderboard 2.0}
\label{table: performance-scenarios-L20}

{\renewcommand{\arraystretch}{1.6}
\begin{tabular}{lccc|lccc} \toprule[2pt]
\textbf{Scenario} & \makecell{\textbf{Route}\\\textbf{Completion (\%)}} &  \makecell{\textbf{Driving}\\\textbf{Score (\%)}} & \makecell{\textbf{Infraction}\\\textbf{Penalty}} & \textbf{Scenario}  & \makecell{\textbf{Route}\\\textbf{Completion (\%)}} & \makecell{\textbf{Driving}\\\textbf{Score (\%)}} & \makecell{\textbf{Infraction}\\\textbf{Penalty}} \\
\hline
Accident & & &
& \makecell[l]{Accident\\TwoWays} & \\ \hline
\makecell[l]{Construction\\Obstacle} & & &
& \makecell[l]{Construction\\ObstacleTwoWays} &  \\ \hline
\makecell[l]{Blocked\\Intersection} & 86.20 & 44.52 & 0.56
& ControlLoss & 95.84 & 64.47 & 0.68 \\ \hline
\makecell[l]{Crossing\\BicycleFlow} & 97.78 & 74.40 & 0.76
& \makecell[l]{DynamicObject\\Crossing} & 81.45 & 54.95 & 0.66 \\ \hline
EnterActorFlow & 99.99 & 80.11 & 0.80
& EnterActorFlowV2 & 99.99 & 96.51 & 0.96 \\ \hline
HazardAtSideLane & 99.99 & 41.67 & 0.42 
& \makecell[l]{HazardAtSideLane\\TwoWays} & 92.62 & 86.26 & 0.92 \\ \hline
HardBreakRoute & 96.39 & 56.92 & 0.60
& HighwayCutIn & 97.60 & 91.03 & 0.93 \\ \hline
HighwayExit & 99.99 & 57.04 & 0.57
& InvadingTurn & 91.53 & 55.94 & 0.64 \\ \hline
\makecell[l]{Interurban\\ActorFlow} & 99.99 & 90.85 & 0.91
& \makecell[l]{InterurbanAdvanced\\ActorFlow} & 99.99 & 57.02 & 0.57 \\ \hline
\makecell[l]{MergerInto\\SlowTraffic} & 99.99 & 75.30 & 0.75
& \makecell[l]{MergerInto\\SlowTrafficV2} & 98.20 & 53.73 & 0.54 \\ \hline
\makecell[l]{NonSignalized\\JunctionLeftTurn} & 97.83 & 48.81 & 0.50
& \makecell[l]{NonSignalized\\JunctionRightTurn} & 97.37 & 54.92 & 0.56 \\ \hline
\makecell[l]{OppositeVehicle\\RunningRedLight} & 98.02 & 83.36 & 0.84
& \makecell[l]{OppositeVehicle\\TakingPriority} & 97.44 & 77.15 & 0.79 \\ \hline
ParkedObstacle & & &
& \makecell[l]{ParkedObstacle\\TwoWays} & \\ \hline
\makecell[l]{ParkingCrossing\\Pedestrian} & 94.52 & 72.63 & 0.74
& ParkingExit & \\ \hline
StaticCutIn & 99.99 & 97.81 & 0.88
& ParkingCutIn & \\ \hline
\makecell[l]{Pedestrian\\Crossing} & 99.32 & 68.26 & 0.69
& PriorityAtJunction & 99.99 & 81.16 & 0.81 \\ \hline
\makecell[l]{SignalizedJunction\\LeftTurn} & 94.56 & 53.90 & 0.56
& \makecell[l]{SignalizedJunction\\RightTurn} & 99.51 & 63.51 & 0.63 \\ \hline
\makecell[l]{VehicleTurning\\Route} & 96.43 & 64.11 & 0.66
& \makecell[l]{VehicleTurning\\RoutePedestrian} & 98.36 & 63.58 & 0.64 \\ \hline
\makecell[l]{VehicleOpensDoor\\TwoWays} & 94.61 & 48.55 & 0.51
& \makecell[l]{YieldTo\\EmergencyVehicle} & 99.99 & 64.36 & 0.64 \\
\bottomrule[2pt]
\end{tabular}
}

\end{table*}

==> tables/scenario-category.tex <==
\begin{table}[htb]
     \centering
     \caption{Rough categorization of scenarios, sorted by difficulty}
     \label{table: scenario-category}
     \begin{tabular}{l|l|l}
      \toprule[2pt] \midrule
      \multirow{2}*{\parbox{1cm}{\textbf{Intuitive}\\\textbf{Strategy}}} & \multirow{2}*{\textbf{Scenario Type}} & \multirow{2}*{\textbf{Specialty}} \\
      & & \\ \midrule
      \multirow{3}*{Keeping} & InterurbanActorFlow \\
      & InterurbanAdvancedActorFlow \\
      & ControlLoss \\ \midrule
      \multirow{11}*{Yielding} & HardBreakRoute & \multirow{5}*{\parbox{2cm}{Threat from\\the front}} \\
      & ParkingCrossingPedestrian \\
      & PedestrianCrossing \\
      & DynamicObjectCrossing \\
      & CrossingBicycleFlow \\ \cmidrule{2-3}
      & HighwayCutIn & \multirow{6}*{\parbox{2cm}{Threat from\\the surrounding}} \\
      & ParkingCutIn \\
      & StaticCutIn \\
      & OppositeVehicleTakingPriority \\
      & OppositeVehicleRunningRedLight \\
      & YieldToEmergencyVehicle \\ \midrule
      \multirow{6}*{Entering} & HighwayExit & \multirow{6}*{Priority sensitive} \\
      & ParkingExit & \\
      & EnterActorFlow & \\
      & EnterActorFlowV2 & \\
      & MergerIntoSlowTraffic & \\
      & MergerIntoSlowTrafficV2 & \\ \midrule
      \multirow{9}*{Turning} & NonSignalizedJunctionRightTurn & Non-signalized; \\
      & NonSignalizedJunctionLeftTurn & priority sensitive \\ \cmidrule{2-3}
      & SignalizedJunctionRightTurn & Signalized; \\
      & SignalizedJunctionLeftTurn &  priority sensitive \\ \cmidrule{2-3}
      & PriorityAtJunction  & \multirow{5}*{Priority sensitive} \\
      & VehicleTurningRoutePedestrian & \\
      & VehicleTurningRoute & \\
      & BlockedIntersection & \\
      & InvadingTurn & \\ \midrule
      \multirow{9}*{Bypassing} & Accident & \multirow{4}*{\parbox{2cm}{Threat from\\the side}} \\
      & ConstructionObstacle & \\
      & HazardAtSideLane & \\
      & ParkedObstacle & \\ \cmidrule{2-3}
      & AccidentTwoWays & \multirow{5}*{\parbox{2cm}{Threat from\\the front}} \\
      & ConstructionObstacleTwoWays & \\
      & HazardAtSideLaneTwoWays & \\
      & ParkedObstacleTwoWays & \\
      & VehicleOpensDoorTwoWays & \\
      \bottomrule[2pt]
     \end{tabular}
 \end{table}
